Multimodal Fusion on Low-quality Data: A Comprehensive Survey

Multimodal fusion focuses on integrating information from multiple modalities with the goal of more accurate prediction, which has achieved remarkable progress in a wide range of scenarios, including autonomous driving and medical diagnosis. However, the reliability of multimodal fusion remains largely unexplored especially under low-quality data settings. This paper surveys the common challenges and recent advances of multimodal fusion in the wild and presents them in a comprehensive taxonomy. From a data-centric view, we identify four main challenges that are faced by multimodal fusion on low-quality data, namely (1) noisy multimodal data that are contaminated with heterogeneous noises, (2) incomplete multimodal data that some modalities are missing, (3) imbalanced multimodal data that the qualities or properties of different modalities are significantly different and (4) quality-varying multimodal data that the quality of each modality dynamically changes with respect to different samples. This new taxonomy will enable researchers to understand the state of the field and identify several potential directions. We also provide discussion for the open problems in this field together with interesting future research directions.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> balance/balanced_mm.tex <==




\section{Balanced Multimodal Learning}
\textcolor{red}{The categorization is not quite clear. While is it possible to reshape the figures to make them more beautiful?}
Different modalities are tightly correlated, since they depict the same concept from different views. This property inspires the flourish of multimodal learning, where multiple modalities are integrated and expected to enhance the understanding of related events or objects. However, despite the natural cross-modal correlation, each modality is with distinct data sources and forms. For instance, audio data is typically represented as one-dimensional waveforms, while visual data consists of images composed of pixels. On the one hand, this discrepancy endows each modality with different learning properties, such as convergence speed, and then makes it is hard to process and learn all modalities well simultaneously, bringing difficulty to joint multimodal learning. On the other hand, this heterogeneity also reflects in the information discrepancy within unimodal data. Even though all modalities depict the same concepts, their information related to the target event or objects are with different amount. For example, considering an audio-visual sample of label \emph{bus}, the visual data apparently show the appearance of the bus, which is easy to be recognized. While the corresponding audio data is a noisy street car sound, whcih is hard to build correlation with the label \emph{bus}. Information amount of visual modality is clearly more than that of audio modality. Due to the greedy nature of deep neural networks, multimodal model would tend to rely on just one modality with sufficient target-related information, while under-fitting the other modalities. To address these challenges and improve the efficacy of multimodal models, recent studies have focused on strategies to balance the differences between modalities and enhance the overall performance of the model.



\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{fig/overfit.pdf}
\caption{The learning curves (error-rate) of audio model (A), video model (V), and the naive joint audio-video (AV) model on Kinetics dataset. Solid lines plot validation error while dashed lines show train error. Figure is from~\cite{wang2020makes}}
\label{fig:discrepancy}
\end{figure}



Discrepancy-oriented methods
In most multimodal models, different modalities are commonly trained jointly with a uniform learning objective. While this joint training strategy has generally proven to be effective in practice, there are still potential risk brought by the discrepancy in data of multiple modalities. The discrepancy of multimodal data in sources and forms result in that each modality has its own learning property. For example, as shown in~\autoref{fig:discrepancy}, in the action recognition dataset Kinetics~\cite{kay2017kinetics}, which contains audio and visual modalities, the audio data tends to require fewer training steps than the vision data before the model begins to overfit~\cite{wang2020deep, feichtenhofer2019slowfast}. The widely-used joint training multimodal framework often neglects this inherent discrepancy of unimodal data, which can potentially lead to negative impacts on the model's performance. More importantly, based on recent study~\cite{wang2020makes}, the jointly trained multimodal model even could be outperformed by the best unimodal counterpart. Thus, it is essential to consider discrepancy in training properties across each modality to improve the performance of the model. To address this issue, several studies have been proposed from different perspective, including learning objective based method, gradient based method and architecture based method.

\subsubsection{Learning-objective-based UML}
Since the jointly trained multimodal framework often only have uniform loss, which integrate the information of all modalities, the learning of each modality is hard to be observed. The learning objective method adds unimodal loss and make it possible to targetedly adjust unimodal training:
\begin{equation}
    \mathcal{L}=\alpha_{mm} \mathcal{L}_{mm} + \alpha_{i} \sum^n_i \mathcal{L}_{i},
\end{equation}
where $\alpha_{mm}$ and $\alpha_{i}$ is the weight of loss function. $n$ is the number of modalities. Since the loss weight determines the influence of corresponding loss function in parameter update, its selection is essential for controlling the unimodal training. Wang \emph{et al.}~\cite{wang2020makes} suggested to determine the optimal loss weights by measuring the proposed overfitting-to-generalization ratio, and could comprehensively consider and balance the discrepancy in convergence speed of each modality.


\subsubsection{Learning rate based UML}
Different from the learning objective based methods that directly introduce unimodal loss, gradient based method pays attention to the back-propagation stage. Considering the discrepancy in convergence speed, learning rate method propose to control the unimodal parameter update by dynamically balancing the learning rates for various modalities~\cite{sun2021learning}:
\begin{equation}
    \theta^i_{t+1} = \theta^i_{t} - \lambda_i g^i_{t},
\end{equation}
where $\lambda_i$ is the learning rate of the parameter of modality $i$ and $g^i_{t}$ is the corresponding gradient. In this way, it is possible to use the modality-specific optimization algorithm for each modality. Specifically, Sun \emph{et al.}~~\cite{sun2021learning} proposed a dynamic approach to balance the learning rates of different modalities by assigning a lower learning rate to the modality that is closer to convergence.



\subsubsection{Architecture-based UML}
Besides the above architecture-agnostic methods which focus on learning objective and learning rate, methods consider the discrepancy in training property problem from the perspective of model architecture are also proposed. At the fusion stage, Xiao \emph{et al.}~\cite{xiao2020audiovisual} proposed to randomly \textcolor{red}{dropping the pathway (more explaination is better)} of the modality with faster convergence speed altogether with certain probability. In this way, the training of corresponding modality is slowed down and its learning dynamics is ensured to be more compatible with other unimodal counterpart. In practice, when the pathway of one modality is dropped during training, its features are often zero-out~\cite{xiao2020audiovisual}. Bedsides the late fusion architecture, studies that utilize low-level cross-modal fusion to enhance multimodal joint learning are also proposed. Zhou \emph{et al}.~\cite{zhou2021joint} utilize central connections to link low-level features in both video and audio streams, capturing spatial (for video frames) and temporal information, thereby achieving high-level semantic representations and improving joint multimodal learning.



\begin{figure}[t]
\centering
\subfigure[Audio.]{\includegraphics[width=0.8\linewidth]{fig/audio.pdf}}
\subfigure[Visual.]{\includegraphics[width=0.8\linewidth]{fig/visual.pdf}}
\caption{Performance of the uni-modal models, joint-trained multimodal model, and multimodal model with OGM-GE~\cite{peng2022balanced} on the validation set of the VGGSound dataset. Figures are from~\cite{peng2022balanced}.}
\label{fig:imbalance}
\end{figure}





\input{balance/table}


\subsection{Imbalance-oriented methods}
The title is not very clear. If possible, please clearly define or describe the two main categories. The above one actually is training oriented, while here it seems "data-oriented or modality-quality-oriented".
In addition to the issue of discrepancy in unimodal training property, even though all modalities convey the same concepts, they contain varying amounts of information related to the target event or objects. Given the inherently greedy nature of deep neural networks, recent studies have further uncovered that multimodal models tend to heavily rely on a single modality that provides sufficient target-related information, while neglecting the others, leading to their under-optimized~\cite{peng2022balanced,huang2022modality}. As shown in Fig.~\ref{fig:imbalance}, Peng \emph{et al.}~\cite{peng2022balanced} empirically verified that the quality of unimodal representations in the multimodal model is worse than that in the corresponding unimodal models, despite the overall superior performance of the multimodal models. Moreover, this under-optimization of each modality is imbalanced. This phenomenon indicates that the learning of each modality in multimodal models is imbalanced. They claim that this imbalanced problem is caused by the model preference for the modality with better performance (i.e., the dominant modality). For instance, the audio modality in the curated sound-oriented dataset, VGGSound~\cite{chen2020vggsound}, is less under-optimized compared to the vision modality. Theoretical analysis conducted by Huang \emph{et al.}~~\cite{huang2022modality} has further confirmed that for the jointly trained multimodal late-fusion framework, the encoder networks can only learn a subset of modalities, and other modalities may fail to be discovered well. This finding is consistent with empirical observations, indicating that the imbalanced preference for different modalities issue needs to be addressed in multimodal learning. To tackle this problem, a series of studies have proposed, encompassing methods based on learning objectives, gradient based techniques, architecture based and data argumentation based methods.


\subsubsection{Learning objective based}
Considering the preference of multimodal model for specific modality, several methods which introduce additional learning objective beyond normal joint learning loss function are proposed. These methods tend to utilize additional loss to break the modality preference of multimodal model. Yang \emph{et al.}~\cite{yang2022mcl} endowed the multimodal contrastive learning loss to constrain the audio and visual modality to be as close as possible in the semantic space, then help to make full use of all modalities. Also paying attention to the multimodal semantic space, Ma \emph{et al}.~\cite{ma2023calibrating} proposed a novel regularization technique Calibrating Multimodal Learning, to enforces the consistency between prediction confidence and the number of modalities, avoiding the issue that multimodal classification models tend to over-rely on specific modalities. In addition to these methods in semantic space, some methods introduce the learning objective of knowledge distillation. Du \emph{et al.}~\cite{du2023uni} proposed to distill the pre-trained uni-modal features to the corresponding parts of multi-modal late-fusion models, to avoid the learning preference for one modality. Differently, Liu \emph{et al.}~\cite{liu2023multimodal} designed self-distillation training strategy, which can automatically teach less-optimized modality from better-optimized modality. Besides these common multimodal classification task, Xu \emph{et al}~\cite{xu2023mmcosine} focused on the audio-visual fine-grained classification task, which have a higher demand for distinguishable feature distribution. They proposed the Multi-Modal Cosine loss, MMCosine, which performs a modality-wise $L2$ normalization to features and weights towards balanced and better multi-modal fine-grained learning.



\subsubsection{Gradient based}
Gradient based methods focus on the back-propagation stage. These methods respectively pay attention to the magnitude and direction of unimodal gradient, to balance the learning of each modality. To slow down the learning of preferred modality and accordingly offer more training efforts to others modalities, Peng \emph{et al.}~\cite{peng2022balanced} proposed an on-the-fly gradient modulation strategy, which dynamically monitors the contribution discrepancy of various modalities to the learning objective during training and mitigates the gradient magnitude of dominant modality to focus more on the under-optimized modality. Inspired by this gradient magnitude modulation idea, Sun \emph{et al.}~\cite{sun2023graph} extended it into the graph-based models of rumor detection task, adaptively adjusting the magnitude of gradients to alleviate the optimization imbalance between modalities. Similarily, Fu \emph{et al.}~\cite{fu2023multimodal} extended the idea of gradient magnitude modulation into audio-visual video parsing task. They further proposed a modality-separated decision unit to well evaluate the unimodal prediction in the more complex audio-visual video parsing framework with more cross-modal interaction. Besides the gradient magnitude, the direction of unimodal gradient is also explored. Fan~\emph{et al.}~\cite{fan2023pmr} suggested that the slow-learning modality’s updating direction is severely
disturbed by the preferred one, making it hard to its training. Subsequently, they utilize prototypes, which are the centroids of each class within the representation space, to refine the updating direction, aiming to improve unimodal performance.





\subsubsection{Architecture based}
The architecture based methods aim to balance the unimodal training by designing better unimodal representation learning modules. He~\emph{et al.}~\cite{he2022multimodal} designed a Multimodal Temporal Attention module, which takes into account the temporal influences of all modalities on each individual unimodal branch. This module facilitates the interaction among unimodal branches and achieves adaptive inter-modal balance. Su \emph{et al.}~\cite{su2023utilizing} focused on the generative scenarios, and utilized the coordinated feature space, named Coordinated Knowledge Mining, to improve the under-optimized modalities with the guidance of preferred modalities. Lin~\emph{et al.}~\cite{lin2023variational} proposes a novel Variational Feature Fusion Module, which regards fusion features as random variables and obtains more balanced segmentation performance for different categories and modalities.



\subsubsection{Data argumentation based}
The data argumentation based methods are with the idea of enhancing more severely under-optimized modality by from the data input stage. The basic intuition is that solely training of unimodal data could avoid the influence of other modalities. There are two kind of strategies, introducing additional individual training for less learnt modality or removing the data of better learnt modality. For the former idea,  Wu \emph{et al.}~\cite{wu2022characterizing} firstly measured the relative speed at which the model learns from one modality compared to other modalities, and then introduce the re-balancing steps at which update the underutilized uni-modal branches intentionally in order to accelerate the model to learn from its input modality. For the latter one, Zhou~\emph{et al.}~\cite{zhou2023adaptive} suggested to adaptively mask the data input of well learnt modality, and accordingly encourage the model to fit other modalities better.


\subsection{Discussion}
Overall, the balanced multimodal learning methods focuses on the learning discrepancy among different modalities, and the model preference for specific modality, which is caused by the heterogeneity of multimodal data. These methods propose solutions from different perspective, including learning objective, gradient, architecture or data argumentation. The balanced multimodal learning is still a sunrise field, with plenty of under-explored directions. Specifically, the current methods mainly limit to the typical multimodal task, mostly discriminative task and a few generative task. In fact, beyond these, the Multimodal Large Language Model, which also need to jointly integrate different modalities, could also suffer from this imbalance problem. It is expected to extend current studies or design new solution in Multimodal Large Language Model settings.



==> balance/balanced_mm_backup.tex <==

\section{Balanced Multimodal Learning}


Different modalities are tightly correlated, since they depict the same concept from different views. This property inspires the flourish of multimodal learning, where multiple modalities are integrated and expected to enhance the understanding of related events or objects. However, despite the natural cross-modal correlation, each modality is with distinct data sources and forms. For instance, audio data is typically represented as one-dimensional waveforms, while visual data consists of images composed of pixels. On the one hand, this discrepancy endows each modality with different learning properties, such as convergence speed, and then makes it is hard to process and learn all modalities well simultaneously, bringing difficulty to joint multimodal learning. On the other hand, this heterogeneity also reflects in the information discrepancy within unimodal data. Even though all modalities depict the the same concepts, their information related to the target event or objects are with different amount. For example, considering an audio-visual sample of label \emph{bus}, the visual data apparently show the appearance of the bus, which is easy to be recognized. While the corresponding audio data is a noisy street car sound, whcih is hard to build correlation with the label \emph{bus}. Information amount of visual modality is clearly more than that of audio modality. Due to the greedy nature of deep neural networks, multimodal model would tend to rely on just one modality with sufficient target-related information, while under-fitting the other modalities. To address these challenges and improve the efficacy of multimodal models, recent studies have focused on strategies to balance the differences between modalities and enhance the overall performance of the model.



\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{fig/overfit.pdf}
\caption{The learning curves (error-rate) of audio model (A), video model (V), and the naive joint audio-video (AV) model on Kinetics dataset. Solid lines plot validation error while dashed lines show train error. Figure is from~\cite{wang2020makes}}
\label{fig:discrepancy}
\end{figure}



\subsection{Discrepancy-oriented methods}


In most multimodal models, different modalities are commonly trained jointly with a uniform learning objective. While this joint training strategy has generally proven to be effective in practice, there are still potential risk brought by the discrepancy in data of multiple modalities. The discrepancy of multimodal data in sources and forms result in that each modality has its own learning property. For example, as shown in~\autoref{fig:discrepancy}, in the action recognition dataset Kinetics~\cite{kay2017kinetics}, which contains audio and visual modalities, the audio data tends to require fewer training steps than the vision data before the model begins to overfit~\cite{wang2020deep, feichtenhofer2019slowfast}. The widely-used joint training multimodal framework often neglects this inherent discrepancy of unimodal data, which can potentially lead to negative impacts on the model's performance. More importantly, based on recent study~\cite{wang2020makes}, the jointly trained multimodal model even could be outperformed by the best unimodal counterpart. Thus, it is essential to consider discrepancy in training properties across each modality to improve the performance of the model. To address this issue, several studies have been proposed from different perspective, including learning objective based method, gradient based method and architecture based method.

\subsubsection{Learning objective based}
Since the jointly trained multimodal framework often only have uniform loss, which integrate the information of all modalities, the learning of each modality is hard to be observed. The learning objective method adds unimodal loss and make it possible to targetedly adjust unimodal training:
\begin{equation}
    \mathcal{L}=\alpha_{mm} \mathcal{L}_{mm} + \alpha_{i} \sum^n_i \mathcal{L}_{i},
\end{equation}
where $\alpha_{mm}$ and $\alpha_{i}$ is the weight of loss function. $n$ is the numbder of modalities. Since the loss weight determines the influence of corresponding loss function in parameter update, its selection is essential for controlling the unimodal training. Wang \emph{et al.}~\cite{wang2020makes} suggested to determine the optimal loss weights by measuring the proposed overfitting-to-generalization ratio, and could comprehensively consider and balance the discrepancy in convergence speed of each modality. 


\subsubsection{Learning rate based}
Different from the learning objective method that directly introduce unimodal loss, gradient based method pay attention to the back-propagation stage. Considering the discrepancy in convergence speed, learning rate method propose to control the unimodal parameter update by dynamically balancing the learning rates for various modalities~\cite{sun2021learning}:
\begin{equation}
    \theta^i_{t+1} = \theta^i_{t} - \lambda_i g^i_{t},
\end{equation}
where $\lambda_i$ is the learning rate of the parameter of modality $i$ and $g^i_{t}$ is the corresponding gradient. In this way, it is possible to use the modality-specific optimization algorithm for each modality. Specifically, Sun \emph{et al.}~~\cite{sun2021learning} proposed a dynamic approach to balance the learning rates of different modalities by assigning a lower learning rate to the modality that is closer to convergence. 



\subsubsection{Architecture based}
Besides the above architecture-agnostic methods which focus on learning objective and learning rate, methods consider the discrepancy in training property problem from the perspective of model architecture are also proposed. At the fusion stage, Xiao \emph{et al.}~\cite{xiao2020audiovisual} proposed to randomly dropping the pathway of the modality with faster convergence speed altogether with certain probability. In this way, the training of corresponding modality is slowed down and its learning dynamics is ensured to be more compatible with other unimodal counterpart. In practice, when the pathway of one modality is dropped during training, its features are often zero-out~\cite{xiao2020audiovisual}. Bedsides the late fusion architecture, studies that utilize low-level cross-modal fusion to enhance multimodal joint learning are also proposed. Zhou \emph{et al}.~\cite{zhou2021joint} utilize central connections to link low-level features in both video and audio streams, capturing spatial (for video frames) and temporal information, thereby achieving high-level semantic representations and improving joint multimodal learning.



\begin{figure}[t]
\centering
\subfigure[Audio.]{\includegraphics[width=0.8\linewidth]{fig/audio.pdf}}
\subfigure[Visual.]{\includegraphics[width=0.8\linewidth]{fig/visual.pdf}}
\caption{Performance of the uni-modal models, joint-trained multimodal model, and multimodal model with OGM-GE~\cite{peng2022balanced} on the validation set of the VGGSound dataset. Figures are from~\cite{peng2022balanced}.}
\label{fig:imbalance}
\end{figure}





\input{balance/table}


\subsection{Imbalance-oriented methods}
In addition to the issue of discrepancy in unimodal training property, even though all modalities convey the same concepts, they contain varying amounts of information related to the target event or objects. Given the inherently greedy nature of deep neural networks, recent studies have further uncovered that multimodal models tend to heavily rely on a single modality that provides sufficient target-related information, while neglecting the others, leading to their under-optimized~\cite{peng2022balanced,huang2022modality}. As shown in~\cite{fig:imbalance}, Peng \emph{et al.}~\cite{peng2022balanced} empirically verified that the quality of unimodal representations in the multimodal model is worse than that in the corresponding unimodal models, despite the overall superior performance of the multimodal models. Moreover, this under-optimization of each modality is imbalanced. This phenomenon indicates that the learning of each modality in multimodal models is imbalanced. They claim that this imbalanced problem is caused by the model preference for the modality with better performance (i.e., the dominant modality). For instance, the audio modality in the curated sound-oriented dataset, VGGSound~\cite{chen2020vggsound}, is less under-optimized compared to the vision modality. Theoretical analysis conducted by Huang \emph{et al.}~~\cite{huang2022modality} has further confirmed that for the jointly trained multimodal late-fusion framework, the encoder networks can only learn a subset of modalities, and other modalities may fail to be discovered well. This finding is consistent with empirical observations, indicating that the imbalanced preference for different modalities issue needs to be addressed in multimodal learning. To tackle this problem, a series of studies have proposed, encompassing methods based on learning objectives, gradient based techniques, architecture based and data argumentation based methods.





\subsubsection{Learning objective based}
Considering the preference of mutlimodal model for specific modality, several methods which introduce additional learning objective beyond norm joint learning loss function are proposed. These methods tends to utilize additional loss to break the modality preference of multimodal model. Yang \emph{et al.}~\cite{yang2022mcl} endowed the multimodal contrastive learning loss to constrain the audio and visual modality to be as close as possible in the semantic space, then help to make full use of all modalities. Also paying attention to the multimodal semantic space, Ma \emph{et al}.~\cite{ma2023calibrating} proposed a novel regularization technique Calibrating Multimodal Learning, to enforces the consistency between prediction confidence and the number of modalities, avoiding the issue that multimodal classification models tend to over-rely on specific modalities. In addition to these methods in semantic space, some methods introduce the learning objective of knowledge distillation. Du \emph{et al.}~\cite{du2023uni} proposed to distill the pre-trained uni-modal features to the corresponding parts of multi-modal late-fusion models, to avoid the learning preference for one modality. Differently, Liu \emph{et al.}~\cite{liu2023multimodal} designed self-distillation training strategy, which can automatically teach less-optimized modality from better-optimized modality. Besides these common multimodal classification task, Xu \emph{et al}~\cite{xu2023mmcosine} focused on the audio-visual fine-grained classification task, which have a higher demand for distinguishable feature distribution. They proposed the Multi-Modal Cosine loss, MMCosine, which performs a modality-wise $L2$ normalization to features and weights towards balanced and better multi-modal fine-grained learning.



\subsubsection{Gradient based}
Gradient based methods focus on the back-propagation stage. These methods respectively pay attention to the magnitude and direction of unimodal gradient, to balance the learning of each modality. To slow down the learning of preferred modality and accordingly offer more training efforts to others modalities, Peng \emph{et al.}~\cite{peng2022balanced} proposed an on-the-fly gradient modulation strategy, which dynamically monitors the contribution discrepancy of various modalities to the learning objective during training and mitigates the gradient magnitude of dominant modality to focus more on the under-optimized modality. Inspired by this gradient magnitude modulation idea, Sun \emph{et al.}~\cite{sun2023graph} extended it into the graph-based models of rumor detection task, adaptively adjusting the magnitude of gradients to alleviate the optimization imbalance between modalities. Similarily, Fu \emph{et al.}~\cite{fu2023multimodal} extended the idea of gradient magnitude modulation into audio-visual video parsing task. They further proposed a modality-separated decision unit to well evaluate the unimodal prediction in the more complex audio-visual video parsing framework with more cross-modal interaction. Besides the gradient magnitude, the direction of unimodal gradient is also explored. Fan~\emph{et al.}~\cite{fan2023pmr} suggested that the slow-learning modality’s updating direction is severely
disturbed by the preferred one, making it hard to its training. Subsequently, they utilize prototypes, which are the centroids of each class within the representation space, to refine the updating direction, aiming to improve unimodal performance.





\subsubsection{Architecture based}
The architecture based methods aims to balance the unimodal training by design better unimodal representation learning modules. He~\emph{et al.}~\cite{he2022multimodal} designed a Multimodal Temporal Attention module, which takes into account the temporal influences of all modalities on each individual unimodal branch. This module facilitates the interaction among unimodal branches and achieves adaptive inter-modal balance. Su \emph{et al.}~\cite{su2023utilizing} focused on the generative scenarios, and utilize the coordinated feature space, named Coordinated Knowledge Mining, to improve the under-optimized modalities with the guidance of preferred modalities. Lin~\emph{et al.}~\cite{lin2023variational} proposes a novel Variational Feature Fusion Module, which regards fusion features as random variables and obtains more balanced segmentation performance for different categories and modalities.



\subsubsection{Data argumentation based}
The data argumentation based methods are with the idea of enhancing more severely under-optimized modality by from the data input stage. The basic intuition is that solely training of unimodal data could avoid the influence of other modalities. There are two kind of strategies, introducing additional individual training for less learnt modality or removing the data of better learnt modality. For the former idea,  Wu \emph{et al.}~\cite{wu2022characterizing} firstly measured the relative speed at which the model learns from one modality compared to other modalities, and then introduce the re-balancing steps at which update the underutilized uni-modal branches intentionally in order to accelerate the model to learn from its input modality. For the latter one, Zhou~\emph{et al.}~\cite{zhou2023adaptive} suggested to adaptively mask the data input of well learnt modality, and accordingly encourage the model to fit other modalities better.


\subsection{Discussion}
Overall, the balanced multimodal learning methods focuses on the learning discrepancy among different modalities, and the model preference for specfic modality, which is caused by the heterogeneity of mutlimodal data. These methods propose solutions from different perspective, including learning objective, gradient, architecture or data argumentation. The balanced multimodal learning is still a sunrise field, with plenty of under-explored directions. Specifically, the current methods mainly limit to the typical multimodal task, mostly discriminative task and a few generative task. In fact, beyond these, the Multimodal Large Language Model, which also need to jointly integrate different modalities, could also suffer from this imbalance problem. It is expected to extend current studies or design new solution in Multimodal Large Language Model settings.



==> balance/balanced_mm_oldversion.tex <==

\section{Balanced Multimodal Learning}
%In multimodal learning, modalities with different information are integrated to enhance the model performance, since multiple modalities depict the same concept from different views and with closely correlated information. Hence, the multimodal models are expected to be superior to the unimodal ones. While the multimodal model generally accomplishes its purpose, there are instances where it falls short and ends up being less effective than the unimodal model~\cite{wang2020makes}. Target to these problem, some researchers hold the perspective that the discrepancy in training properties or model preference suppress the potential of multimodal learning. On the one hand, data of different modalities have heterogeneous source and form, which could bring natural discrepancy for the training of multimodal data. For example, audio data is often one-dimension waveform while vision data are images composed by pixels. On the other hand, the discriminative information of each modality to the target label also have discrepancy. For instance, for an audio-visual sample \emph{blowing wind}, vision is naturally less discriminative than auditory. Therefore, the multimodal modal could tend to have preference for the audio modality in this case. Therefore, a series of studies have emerged in recent years to balance these unimodal discrepancy and improve the ability of multimodal model.

\input{balance/table}

In multimodal learning, modalities with different information are integrated to enhance the model performance, since multiple modalities depict the same concept from different views and with closely correlated information. Hence, the multimodal models are expected to be superior to the unimodal ones. While the multimodal model generally accomplishes its purpose, there are instances where it falls short and ends up being less effective than the unimodal model~\cite{wang2020makes}. To address this issue, some researchers argue that the differences in training properties or model preferences could hinder the potential of multimodal learning. On the one hand, the widely used jointly training multimodal data strategy could not handle the heterogeneity of modalities with different data sources and forms. For instance, audio data is typically represented as one-dimensional waveforms, while visual data consists of images composed of pixels. On the other hand, each modality may contribute different amounts of discriminative information towards the target label. For instance, for an audio-visual sample~\emph{blowing wind}, vision is naturally less discriminative than auditory. Therefore, the multimodal model could tend to have a preference for the audio modality in this case. To address these challenges and improve the efficacy of multimodal models, recent studies have focused on strategies to balance the differences between modalities and enhance the overall performance of the model.



\subsection{Balance training properties of modalities}
%In most multimodal models, different modalities are trained jointly with a uniform learning objective. Although the widely used joint training strategy indeed works well in most cases, the heterogeneous training properties of unimodal data are often ignored, which could bring potential negative impact. Based on recent studies, various modalities tend to converge at different rates~\cite{wang2020deep, feichtenhofer2019slowfast}. Take the action recognition dataset, Kinetics-400~\cite{kay2017kinetics} containing audio and vision modality, as an example, the audio data requires fewer training steps before the model starts to overfit than the vision data~\cite{wang2020deep, feichtenhofer2019slowfast}. Therefore, it is necessary to balance the training properties of each modality. 

In most multimodal models, different modalities are commonly trained jointly with a uniform learning objective. While this joint training strategy has generally proven to be effective in practice, it often neglects the inherent differences in the training properties of unimodal data, which can potentially lead to negative impacts on the model's performance. Recent studies have revealed that various modalities may converge at different rates~\cite{wang2020deep, feichtenhofer2019slowfast}. For example, in the action recognition dataset Kinetics-400~\cite{kay2017kinetics}, which contains audio and visual modalities, the audio data tends to require fewer training steps than the vision data before the model begins to overfit~\cite{wang2020deep, feichtenhofer2019slowfast}. Thus, it is essential to consider the balancing of training properties across each modality to improve the performance of the model.

%To alleviate this problem, Wang et al.~\cite{wang2020makes} proposed to introduce additional uni-modal loss functions besides the multimodal objective and find the optimal loss weight by measuring the overfitting-to-generalization ratio. With similar motivation, Xiao et al.~\cite{xiao2020audiovisual} utilized a simple method of randomly dropping the modality with a faster learning pace during training and making its learning more compatible with other modalities, to balance the jointly multimodal training. From the perspective of optimization, Sun et al.~\cite{sun2021learning} proposed to dynamically balance the learning rates of different modalities, by assigning lower learning late to the modality closer to convergence. 

To address the issue of imbalanced training properties in multimodal learning, several recent studies have proposed various approaches. Wang et al.\cite{wang2020makes} suggested the incorporation of additional uni-modal loss functions in addition to the multimodal objective, with optimal loss weights determined by measuring the overfitting-to-generalization ratio. With similar motivation, Xiao et al.\cite{xiao2020audiovisual} proposed a simple method of randomly dropping the modality with a faster learning rate during training and ensuring its learning is more compatible with other modalities to balance the jointly multimodal training. From the optimization perspective, Sun et al.~\cite{sun2021learning} proposed a dynamic approach to balance the learning rates of different modalities by assigning a lower learning rate to the modality that is closer to convergence. 

Overall, these methods focus on the discrepancy in training properties of different modalities, to balance joint multimodal training.



\subsection{Balance model preference of modalities}


In addition to the issue of imbalanced training properties, recent research has uncovered that multimodal models can exhibit imbalanced preference for different modalities, resulting in under-optimized with different degree unimodal representations within the jointly trained multimodal model~\cite{peng2022balanced,huang2022modality}. Experimental results reported by Peng et al.\cite{peng2022balanced} suggest that the quality of unimodal representations in the multimodal model is worse than that in the corresponding unimodal models. Moreover, this under-optimization of each modality is imbalanced, despite the overall superior performance of the multimodal models. This phenomenon indicates that the learning of each modality in multimodal models is imbalanced. They claim that this imbalanced problem is caused by the model preference for the modality with better performance (i.e., the dominant modality). For instance, the audio modality in the curated sound-oriented dataset, VGGSound~\cite{chen2020vggsound}, is less under-optimized compared to the vision modality. Theoretical analysis conducted by Huang et al.~\cite{huang2022modality} has further confirmed that for the jointly trained multimodal late-fusion framework, the encoder networks can only learn a subset of modalities, and other modalities may fail to be discovered. This finding is consistent with empirical observations, indicating that the imbalanced preference for different modalities issue needs to be addressed in multimodal learning.


%Besides the discrepancy in training properties, some researchers further discovered that multimodal models have imbalanced preference for different modalities, and the unimodal representation in the jointly trained multimodal model is often under-optimized with different degree~\cite{peng2022balanced,huang2022modality}. Experimentally, Peng et al.~\cite{peng2022balanced} observed that the quality of unimodal representation in the multimodal model is clearly worse than that in the unimodal models, and more importantly, this under-optimized degree of each modality is imbalanced, although the multimodal models outperform its unimodal counterparts. This phenomenon indicates that the learning of multimodal model for each modality is imbalanced. They claim that this imbalanced problem is caused by the model preference for the modality with better performance (i.e., the dominant modality). For instance, the audio modality in the curated sound-oriented dataset, VGGSound~\cite{chen2020vggsound}, is less under-optimized compared to the vision modality. Theoretically, Huang et al.~\cite{huang2022modality} proved that for the jointly trained multimodal late-fusion framework, the encoder networks could only learn a subset of modalities and other modalities would fail to be discovered, which is consistent with the empirical observation. 


%To balance the learning of multimodal model for each modality and ease the model preference for the dominant modality, the optimization process of each modality is regulated by Peng et al.~\cite{peng2022balanced} through the use of an on-the-fly gradient modulation strategy. This involves dynamically monitoring the contribution discrepancy of various modalities to the learning objective during training and adapting the gradients to focus more on the under-optimized modality. Du et al.~\cite{du2021improving} proposed a distillation method to distil the pre-trained unimodal features to the multi-modal networks for alleviating the insufficient feature learning problem in the multimodal model. Wu et al.~\cite{wu2022characterizing} measured the speed at which the model learns from one modality relative to the other modalities, and then proposed to guide the model to learn from previously underutilized modalities. More recently, according to Xu et al.~\cite{xu2023mmcosine}, the previously mentioned methods for addressing imbalances between modalities often struggle with more fine-grained multimodal tasks. As a solution, they introduce MMCosine, a multi-modal cosine loss that performs modality-wise L$2$ normalization on features and weights to promote more balanced and effective learning for these tasks.


To balance the learning of each modality in multimodal models and overcome the model preference for the dominant modality, various methods have been proposed~\cite{peng2022balanced,wu2022characterizing,xu2023mmcosine,zhou2023adaptive}. Peng et al.\cite{peng2022balanced} proposed an on-the-fly gradient modulation strategy, which dynamically monitors the contribution discrepancy of various modalities to the learning objective during training and mitigates the gradients of dominant modality to focus more on the under-optimized modality. Du et al.\cite{du2021improving} proposed a distillation method to alleviate this under-optimized unimodal representation learning problem in the multimodal model by distilling the pre-trained unimodal features to the multi-modal networks. To alleviate the model preference issue, Wu et al.\cite{wu2022characterizing} measured the relative speed at which the model learns from one modality compared to other modalities and proposed a method to guide the model to learn from previously underutilized modalities. Recently, according to Xu et al.\cite{xu2023mmcosine}, these methods often struggle with more fine-grained multimodal tasks. To address this, they introduced MMCosine, a multi-modal cosine loss that performs modality-wise L$2$ normalization on features and weights to promote more balanced and effective learning for these tasks.

%To provide data preparation for the imblanced model preference problem, Xia et al.~\cite{xia2023balanced} build a balanced audiovisual dataset, with uniformly distributed modality discrepancy over the whole dataset, which could be used to better evaluate imbalance algorithms.

In a nutshell, these methods analyze and alleviate the imbalanced multimodal model preference for different modalities from various perspective, improving the learning of multimodal model for each modality. 


==> dynamic/notations.tex <==
\begin{table*}[htbp]
\setlength{\abovecaptionskip}{0.0cm}  %段前
\setlength{\belowcaptionskip}{0.0cm} %段后
\vspace{-0.0cm}
% \vskip 0.35in
\begin{center}
%\begin{spacing}{1.05}   
\caption{A summary of the notations we mainly used in multimodal fusion \label{notations}.}
\center
{
\setlength{\tabcolsep}{1.9mm}
\begin{tabular}{cc}
\toprule
    \multirow{1}{*}{$\mathbf{x}=[x^1,\cdots,x^m]$}  & \multirow{1}{*}{multimodal input consists of $m$ modalities} 
\\\multirow{1}{*}{$\mathcal{X}=\mathcal{X}^1\times\cdots\times\mathcal{X}^m$}  & \multirow{1}{*}{multimodal input space consists of $m$ unimodal space} 
\\
    \multirow{1}{*}{$y\in \mathcal{Y}$}  & \multirow{1}{*}{target $y$ and corresponding space $\mathcal{Y}$}  \\
                            \multirow{1}{*}{$\mathbf{z}\in \mathcal{Z}$}  & \multirow{1}{*}{multimodal latent representation $\mathbf{z}$ and latent space $\mathcal{Z}$}\\ \multirow{1}{*}{$h:\mathcal{X}\rightarrow \mathcal{Z}$}  & \multirow{1}{*}{multimodal fusion mapping}  \\ \multirow{1}{*}{$g:\mathcal{Z}\rightarrow \mathcal{Y}$}  & \multirow{1}{*}{task-specific mapping}  \\ \bottomrule
 \\
\end{tabular}}
% \end{spacing}
\end{center}
\end{table*}





==> incomplete/incomplete_backup.tex <==
\section{Incomplete multimodal Learning}
The collected multimodal data in real applications are often incomplete with partial missing modalities for some samples due to unexpected factors, such as equipment damage, data transmission and storage loss. For a concrete example, in recommendation system, the browsing behavior history and credit score information may not always be available for some users \cite{shao2013clustering}. Similarly, multimodal data can be highly incomplete in medical analysis due to the patients' personal preferences, economic constraints and limitation in medical resources. For example, although combining data from multiple modalities e.g., magnetic resonance imaging (MRI) scans, positron emission tomography (PET) scans, and cerebrospinal fluid (CSF) information can obtain a more accurate diagnosis for Alzheimer's Disease \cite{zhang2012multi,liu2014inter}, owing to high measurement cost for PET scans and uncomfortable invasive tests for CSF, some patients may refuse to conduct these examinations. Thus, incomplete multimodal data commonly exist in Alzheimer's Disease diagnosis \cite{thung2014neurodegenerative}. Typically, conventional multimodal learning models assume the completeness of multimodal data and thus cannot be applied to partial missing modalities directly. For this issue, incomplete multimodal learning, aiming at exploring information of incomplete multimodal data with partial missing modalities, appears and has received increasing research interests in recent years \cite{wen2022survey}. In this section, we mainly focus on the current progress of researches on incomplete multimodal learning. From the view of whether to impute the missing data or not, we categorize existing methods into two groups including imputation-based and imputation-free incomplete multimodal learning, where the imputation based methods are further divided into two groups as shown in Fig.~\ref{fig:incomdata} including instance and modality level imputation.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\textwidth]{fig/imputation.png}
    \caption{\textbf{Imputation based incomplete multimodal learning.}} 
    \label{fig:incomdata}
\end{figure*}

\subsection{Imputation based incomplete multimodal learning}
For the incomplete multimodal data, a natural approach to address the missing modality learning issue is to directly impute the missing modalities or related missing information in the kernels or graphs constructed from the data as shown in Fig.~\ref{fig:incomdata}. Then the conventional multimodal learning algorithm can be applied to downstream tasks. In this branch, the existing imputation-based works can be further divided into two categories, including model-agnostic imputation and model-specific imputation. The model-specific imputation methods generally design a imputation model or network for missing data recovery while the imputation model is not necessary for the model-agnostic imputation methods which usually utilizes heuristic filling strategy for the missing modalities.

\subsubsection{Model-agnostic imputation}
For the missing modalities, the simplest imputation schemes are zero imputation and mean value imputation, i.e., filling missing values with zero or imputation with the averaged value in the corresponding modality, which is widely used as the baseline methods in most studies \cite{shao2015multiple,zhao2016incomplete}. However, previous work~\cite{shao2015multiple} shows that the naive imputation may lead to unpromising performance. To address this issue, a weighted matrix factorization model is proposed to assign small weights for the imputed modalities, mitigating the negative influence on optimization \cite{shao2015multiple}. Furthermore, for an online multimodal clustering case, a dynamic weighting and imputation mechanism is designed according to the valid modalities and task at hand\cite{shao2016online}. To implement the graph-based approach on incomplete multimodal data, Wang \emph{et al}.~\cite{wang2019spectral} utilize similarity values computed from valid modalities to impute the missing elements of graph. In \cite{gao2016incomplete}, the missing elements in the incomplete kernels are pre-imputed by the average of all columns. In \cite{zhou2019consensus}, the authors also utilize the average instance of the corresponding modality to impute the missing instances and then assign a small weight to those imputed instances during the graph construction phase.

\subsubsection{Learning based imputation}
For the learning based imputation, according to the filling values, we can further divide it into two categories: kernel/graph-based imputation and raw data imputation.

\textbf{Kernel/graph-based imputation}: Kernel and graph learning based approaches are two main lines of incomplete multimodal learning, which transform the learning phase from the raw data to the kernel space or graph. For the kernel and graph constructed from each modality, each element represents the relationship in kernel space or affinity/similarity of instance pairs. The partial missing instances in each modality result in incomplete kernels and graphs. A line of works has been proposed to address the incomplete kernel/graph-based multimodal learning issue. Here we highlight a few seminal works. David Williams \emph{et al}.~\cite{williams2005analytical} proposed a Gaussian mixture model based method that can analytically compute the missing Gaussian kernel elements associated with the missing instances. Trivedi \emph{et al}.~\cite{trivedi2010multiview} proposed a kernelized canonical correlation analysis (KCCA) based imputation method, which minimizes a Laplacian kernel regularization to obtain the missing kernel elements. Although effective, it is only applicable to the two-modal data with one complete modality. Lately, collective kernel learning (CKL)~\cite{shao2013clustering} is proposed to mutually complete the two incomplete kernels associated with the two incomplete modalities. For the data with more than two modalities, such as the case with $k$ modalities ($k \ge 3$), CKL needs to recover each kernel matrix ${K_{i + 1}}$ of the $\left( {i + 1} \right)$th modality according to kernel ${K_i}$ in a cycle iteration scheme. Sahely \emph{et al}.~\cite{bhadra2017multi} proposed a multimodal kernel completion method based on the sparse reconstruction technique. The method can complete the missing rows and columns of all kernels jointly in a within-kernel preservation and between-kernel exploration framework. Yang \emph{et al}.~\cite{yang2018semi} reduced incomplete multi-modal imputation into semi-supervised learning problem. They further proposed SLIM (Semi-supervised Learning with Incomplete Modality ) and its kernel vision SLIM-K based on matrix completion for solving the modal incompleteness. Recently, Liu \emph{et al}. proposed several flexible kernel methods to recover the missing kernel elements for incomplete multimodal clustering tasks~\cite{liu2019multiple,ye2017consensus,zhu2018localized,liu2021incomplete}. For instance, MKKM-IK~\cite{liu2019multiple} unifies the kernel completion and consensus partition matrix learning in a unified framework: 
\begin{equation}\label{im_eq1}
\begin{array}{l}
\mathop {\min }\limits_{H,\gamma ,\left\{ {{K^{\left( m \right)}}} \right\}_{m = 1}^l} \text{\rm Tr}\left( {\sum\limits_{}^{} {\gamma _m^2{K^{\left( m \right)}}\left( {I - H{H^T}} \right)} } \right)\\
s.t.HH = I,\sum\nolimits_{m = 1}^l {{\gamma _m}}  = 1,0 \le \gamma  \le 1,\\
\forall \left\{ {i,j} \right\} \in {\Omega ^{\left( m \right)}},K_{i,j}^{\left( m \right)} = {\kappa ^{( m)}}\left( {x_i^{\left( m \right)},x_j^{\left( m \right)}} \right),
\end{array}
\end{equation}
where ${\kappa ^{\left( m \right)}}$ denotes the kernel function for the $m$-th modality. ${\Omega ^{\left( m \right)}}$ denotes the set of location index corresponding to the un-missing instance in the $m$-th modal. ${K^{\left( m \right)}} \in {R^{n \times n}}$ represents the kernel of the $m$-th modality to recover, in which some elements $K_{i,j}^{\left( m \right)}$ corresponding to the observed instances in the $m$-th modality are unchanged during the optimization. $H \in {R^{n \times c}}$ is the consensus partition matrix for data clustering.

By aligning all incomplete kernels to a consensus kernel derived from the consensus orthogonal representation, these methods can jointly obtain the missing elements associated with missing instances and the consensus partition representation shared by all modalities for incomplete multimodal data clustering. Besides of kernel-based methods, an adaptive graph completion method is developed to recover the missing similarities of all graphs with respect to all modalities~\cite{wen2020adaptive}. The method mainly employs the sparse-representation-based data reconstruction technique to borrow the graph information of other modalities in recovering the missing elements of each modality.

\textbf{Raw data imputation}: Some methods recover the missing modalities at raw feature level. For example, VIGAN (View Imputation via Generative Adversarial Network)~\cite{shang2017vigan} is a pioneering work based on generative adversarial network (GAN) and Autoencoder for missing modality recovery. VIGAN employs GAN to initialize the missing modality according to another modality of the same sample and then uses denoise Autoencoder to refine the recovered missing modalities. A limitation of VIGAN is that it is not applicable to data with more than two modalities. Subsequently, partial multimodal clustering via consistent GAN (PMVC\_CGAN) \cite{wang2018partial} and adversarial incomplete multimodal clustering (AIMC) \cite{xu2019adversarial} are proposed for missing modality imputation and incomplete multimodal clustering. Different from VIGAN which uses one available data to generate the corresponding missing modality, PMVC\_CGAN and AIMC seek to learn the missing modalities from the common representation encoded by the un-missing modalities of the same sample. In~\cite{arya2021generative}, a two-stage incomplete deep multimodal network is proposed for breast cancer prediction. Similar to the network structures of AIMC and PMVC\_CGAN, GAN is introduced to enhance the quality of missing view imputation. Besides of GAN-based methods, CRA (cascaded residual autoencoder) stacks all modalities into one modal and treats the missing modalities imputation as conventional missing feature completion by optimizing a single-modal cascaded residual autoencoder network \cite{tran2017missing}. Liu \emph{et al}.~\cite{Liu2023Information} proposed another representative autoencoer based imputation framework termed RecFormer for clustering task. Specifically, RecFormer employs a two-stage autoencoder network with the self-attention structure to synchronously extract high-level semantic representations and recover the missing data

To obtain a more reliable modality imputation performance, Tang \emph{et al}.~\cite{tang2022deep} proposed to impute the modality as the average of corresponding semantic neighbors. Lin \emph{et al}.~\cite{lin2022dual} established a dual prediction model that can predict the latent representation of the missing modality according to that of the observed modality and then used the decoder to obtain the recovered missing modality according to the predicted latent representation. matrix factorization is also applied for raw modality imputation. For example, UEAF (Unified Embedding Alignment Framework)~\cite{wen2019unified} and IMCRV (Incomplete multimodal Clustering with Reconstructed Views)~\cite{yin2021incomplete} provide two matrix factorization based missing modality recovery models, which can reversely reconstruct the data of missing modalities from the common representation. In~\cite{wen2021unified}, low-rank representation and tensor learning are introduced for joint missing modality recovery and graph completion. Explicitly taking the reliability of imputation into account, Xie \emph{et al}.~\cite{xie2023exploring} introduced the Uncertainty-induced Incomplete Multi-View Data Classification (UIMC) model to address challenges in classifying incomplete multi-view data with missing perspectives. UIMC explores and exploits uncertainty by imputing missing modalities as distributions rather than deterministic values, allowing for more reliable predictions. The model employs an evidential multimodal learning framework to weigh imputed data, reducing the impact of low-quality imputations. In incomplete multimodal action recognition task, Sangmin \textit{et al.} proposed a modular network called ActionMAE, which randomly drops modality features and then learn to impute them.

Lin \emph{et al}. proposed a novel objective by integrating representation learning and data recovery into a unified information-theoretic framework termed COMPLETER~\cite{lin2021completer} for clustering task. Specifically, COMPLETER propose to learn intra-modal consistency by maximizing mutual information and learn modal imputation by minimizing conditional entropy. Dong \emph{et al}. proposed a deep Gaussian processes model to impute the missing modalities and further enhance the performance of downstream tasks~\cite{dong2023partial}. Motivated by contrastive learning, Yang \emph{et al}. introduced a multimodal imputation paradigm termed SURE for robust multimodal imputation~\cite{yang2022robust}. The method treats complete multimodal pairs as positive and randomly sampling unpaired samples as negative. A noise-robust contrastive loss is employed to alleviate the influence of false negatives. Li \emph{et al}. proposed a prototype-based multimodal imputation method, which incorporates a two-stream model with dual attention layers and contrastive learning mechanism to learn modal-specific prototypes and model the cross-modal relationship~\cite{li2023incomplete}. Considering incomplete multimodal inputs, the model performs modality imputation using prototypes learned from the incomplete multimodal training data and the sample-prototype relationship inherited from the observed modalities. Xu \emph{et al}.~\cite{ren2024novel} proposed a novel federated multi-view clustering method using an unsupervised technique to evaluate and refine imputation quality, efficiently handling various scenarios of incomplete multi-view data.

\subsection{Imputation-free incomplete multimodal learning}
Different from the above imputation based methods, imputation-free methods only focus on exploring the information corresponding to the available modalities. Most of the related imputation-free methods can be grouped into four mainstreams: latent representation and projection learning, graph learning, kernel learning, and deep learning.
\subsubsection{Latent representation and projection learning}
Latent representation and projection learning based incomplete multimodal learning (taking clustering for example) generally seek to obtain a multimodal latent representation by exploring the available partially aligned information among these available modalities. In this branch, partial multimodal clustering (PMVC)~\cite{li2014partial} is a popular and pioneering work based on matrix factorization. It concentrates on encoding the data with two fully observed modalities into a common representation within the latent subspace. Based on PMVC, incomplete multimodal grouping (IMG) \cite{zhao2016incomplete} and partial multimodal subspace clustering \cite{xu2018partial} further introduce the graph constraints to capture the structure information in the latent common subspace. A basic model used in the above methods to learn the latent common representation from the incomplete bi-modal data can be formulated as follows:
\begin{equation}\label{im_eq2}
\begin{array}{l}
\mathop {\min }\limits_{{P_o},\left\{ {P_{uo}^{\left( m \right)},{U^{\left( m \right)}}} \right\}_{m = 1}^2} \sum\limits_{m = 1}^2 {\left\| {\left[ \begin{array}{l}
X_o^{\left( m \right)}\\
X_{uo}^{\left( m \right)}
\end{array} \right] - \left[ \begin{array}{l}
{P_o}\\
P_{uo}^{\left( m \right)}
\end{array} \right]{U^{\left( m \right)}}} \right\|_F^2} \\
{\kern 80pt}   + \Psi \left( {{P_o},P_{uo}^1,P_{uo}^2,{U^1},{U^2}} \right),
\end{array}
\end{equation}
where ${X^{(1)}} = \left[ \begin{array}{l}
X_o^{(1)}\\
X_{uo}^{(1)}
\end{array} \right]$ and ${X^{(2)}} = \left[ \begin{array}{l}
X_o^{(2)}\\
X_{uo}^{(2)}
\end{array} \right]$ denote the data in the two modalities, respectively. ${X_o} = \left\{ {X_o^{(1)},X_o^{(2)}} \right\}$ denotes the samples with two fully observed modalities. $X_{uo}^{(1)}$ and $X_{uo}^{(2)}$ are the data with only the first modality and second modality, respectively. $U^1$ and $U^{(2)}$ are the basis matrices. $\Psi \left( {{P_o},P_{uo}^{(1)},P_{uo}^{(2)},{U^{(1)}},{U^{(2)}}} \right)$ denotes the constraints on these variables. The learned common representation can be represented as $P = \left[ {{P_o};P_{uo}^{(1)};P_{uo}^{(2)}} \right]$.

Zhou \emph{et al}.~\cite{zhou2019latent} integrated the latent representation learning and regression into a unified framework for Alzheimer's disease diagnosis based on incomplete multimodal neuroimaging and genetic data. The motivation of the latent representation learning module for incomplete multimodal data is similar to model (\ref{im_eq2}). However, a widely recognized limitation of the above methods based on model (4) is that they are only applicable to the case with bi-modal data. To address this limitation, weighted matrix factorization is introduced, where doubly aligned incomplete multimodal clustering \cite{hu2018doubly}, one-pass incomplete multimodal clustering \cite{hu2019one}, and localized sparse incomplete multimodal clustering \cite{liu2023localized} are representative methods. These models generally impose the location information of missing instances as the weighted matrices with binary values on the matrix factorization model to eliminate the loss yet reduce the negative influence of the missing instances. The basic model of the weighted matrix factorization based methods can be formulated as follows:
\begin{equation}\label{im_eq3}
\mathop {\min }\limits_{{U^{(m)}},P} \sum\limits_{m = 1}^M {\left\| {{W^{(m)}}\left( {{X^{(m)}} - P{U^{(m)}}} \right)} \right\|_F^2 + \Psi \left( {{U^{(m)}},P} \right)},
\end{equation}
where ${{X^{(m)}}}$ denotes the data of the $m$-th modality with missing instances being 0 or the average value of the available instances in the modality. ${{U^{(m)}}}$ denotes the basic matrix and ${\Psi \left( {{U^{(m)}},P} \right)}$ denotes the constraints of these variables. $P$ is the latent complete common representation to learn. $W^{(m)}$ is a diagonal matrix constructed according to the instance missing location information in the $m$-th modality. For example, if the $i$-th sample does not have the $m$-th modality, then $W_{i,i}^{(m)}$ can be simply set as 0, otherwise $W_{i,i}^{(m)}=1$. With such a setting, the negative influence of missing modalities can be eliminated from the learning model, and the available aligned consistent and complementary information can be explored for the latent common representation learning.

Compared with the basic model (\ref{im_eq2}), the methods based on model (\ref{im_eq3}) are more flexible and can be easily extended to the data with more than two modalities and arbitrary incomplete cases. Besides of these weighted matrix factorization models, a generalized incomplete multimodal clustering model is proposed to learn a complete common representation from the incomplete modal-specific representations with a partially aligned learning term \cite{wen2020generalized}. Specifically, such a partially aligned learning term can be regarded as a variant of the weighted common representation learning. To prevent the model from overly focusing on certain modalities with larger dimensions, projective incomplete multimodal clustering transforms the matrix factorization into a variant of the weighted projection learning model to obtain the consensus representation from the incomplete multimodal data \cite{deng2023projective}. For the incomplete multimodal and incomplete multi-label classification task, a variant of the weighted projection learning model \cite{li2021concise} and weighted matrix factorization model \cite{tan2018incomplete} are developed to explore the information of available modalities. In terms of infant neuroscience, Zhang \emph{et al}. propose to explore incomplete multimodal data by constructing a latent representation to capture the complementary information from incomplete time-points~\cite{zhang2018infant}. In summary, the above methods focus on exploring the available information of the observed modalities by introducing some techniques like the weighting mechanism to eliminate the loss of those missing modalities.

\subsubsection{Graph learning based}
Graph learning based method is very popular in conventional multimodal clustering. This technique is also widely considered and integrated into other methods like matrix factorization based and deep learning based methods, to explore the structure information of data so as to enhance the performance. For incomplete multimodal learning, the main challenges to apply the graph learning based approach are two-folds: (1) How to obtain the intrinsic structure relationships among the available instances in each modality? (2) How to fully explore these incomplete relationships? For example, for the incomplete multimodal clustering tasks, one of the major challenges is to obtain the consensus complete graph or representation from these incomplete modal-specific relationships associated with all incomplete modalities. Specifically, we can formulate this issue as the following simple framework:
\begin{equation}\label{im_eq4}
\mathop {\min }\limits_{\left\{ {{S^{\left( m \right)}}} \right\}_{m = 1}^l,Z} \sum\limits_{m = 1}^l {f\left( {{{\bar X}^{\left( m \right)}},{S^{\left( m \right)}}} \right) + g\left( {{S^{\left( m \right)}},{W^{\left( m \right)}},Z} \right)},
\end{equation}
where ${{{\bar X}^{\left( m \right)}}}$ denotes the set of the available instances in the $m$-th modality. ${{S^{\left( m \right)}}}$ represents the modal-specific graph learned from the $m$-th modal data ${{{\bar X}^{\left( m \right)}}}$. ${{W^{\left( m \right)}}}$ is the modal-available or missing indicator matrix as defined in Eq.~\ref{im_eq3}. Taking the incomplete multimodal clustering task for example, the target of general graph learning based method is to learn the consensus graph or representation $Z$ from the incomplete data $\left\{ {{{\bar X}^{\left( m \right)}}} \right\}_{m = 1}^l$ or graph $\left\{ {{S^{\left( m \right)}}} \right\}_{m = 1}^l$, such that a consensus clustering result can be obtained by performing k-means or spectral clustering on $Z$. 

As one representative work, incomplete multimodal spectral clustering~\cite{wen2018incomplete} proposed a unified framework that integrates the adaptive collaborative representation based modal-specific graph learning and co-regularized consensus representation learning. The first term enables the method to adaptively capture the intrinsic relationships among available instances of each modality and the second term seeks to obtain the consensus complete representation by fully exploring such similarity relationship. For the data with only two modalities, Wu \emph{et al}.~\cite{wu2018incomplete} proposed a method based on structured graph learning, which seeks to learn two modal-specific graphs corresponding to the two modalities with a partially aligned constraint on the samples with complete modalities. Then, the method obtains the modal-specific clustering from the two graphs and adopts the best one-to-one map to obtain the final consensus clustering result. The work in \cite{wen2023highly} pre-constructs several modal-specific graphs from the available instances of every modality and then learns a consensus graph from these graphs via a weighted consensus graph learning model with the constraint of pre-constructed confident neighbor information. In summary, except for the imputation based graph methods, most graph-based incomplete multimodal learning methods seek to exploit certain similarity information among available instances to discover the clustering structure and clustering result. In \cite{xiang2013multi}, for Alzheimer's disease prediction, a unified linear regression based model is developed, in which the incomplete multimodal data are segmented into several complete subsets for model optimization. Similar to the above method, Liu \emph{et al}.~\cite{liu2017view} segmented the incomplete multimodal data into several complete subsets and used the sparse representation algorithm to construct the sub-graphs from these subsets. Then a modal-aligned hypergraph learning model is developed to perform the Alzheimer's disease diagnosis.

\subsubsection{Kernel learning based}
Kernel learning based methods transform the learning phase from the raw-feature space into the kernel space. Similar to the graph learning based methods, each element of the kernel matrix denotes a kind of the similarity or connection values of the corresponding two samples. For incomplete multimodal data, the constructed kernels w.r.t. different modalities will also be incomplete with missing rows and columns. Thus, the target of kernel learning based methods for incomplete multimodal data is to explore the information of these incomplete kernels. In this branch, most methods consider kernel imputation as we mentioned above like model (\ref{im_eq1}) while relatively few works focus on exploiting certain available kernel information. Late fusion incomplete multimodal clustering~\cite{liu2018late} is one of the representative kernel imputation-free methods for incomplete multimodal data. The method does not need to impute the missing kernel elements but tries to simultaneously impute the missing representations corresponding to the missing modalities and learn the consensus representation in a joint framework. Furthermore, to reduce the low-quality imputation of the latent representations, Liu \emph{et al}.~\cite{liu2020efficient} proposed an efficient and effective regularized incomplete multimodal clustering method (EERIMVC), which integrates the initialized consensus representation as prior knowledge. In this model, such prior representation is obtained by the conventional complete kernel algorithm with zero or average filling. Therefore, the quality of the initialized consensus representation will be an important factor to the performance. To break the gap between representation learning and label prediction, a one-stage incomplete multimodal clustering method is proposed \cite{zhang2021one}. Compared with EERIMVC, this method replaces the consensus representation with a clustering label matrix and an orthogonal matrix. 

To sum up, for the incomplete multimodal raw data $\left\{ {{X^{\left( m \right)}} \in {R^{{d_m} \times n}}} \right\}_{m = 1}^l$ or derived incomplete kernel data $\left\{ {{K^{\left( m \right)}} \in {R^{n \times n}}} \right\}_{m = 1}^l$ with a binary matrix $W \in {\left\{ {0,1} \right\}^{n \times l}}$ indicating the location of missing modalities, the late fusion based kernel methods generally seek to learn the consensus representation $P \in {R^{n \times c}}$ from the initialized representations $\left\{ {{{\bar P}^{\left( m \right)}} \in {R^{{n_m} \times c}}} \right\}_{m = 1}^l$ of the available modalities as follows:
\begin{equation}\label{im_eq5}
\begin{array}{l}
\mathop {\max }\limits_{\phi \left( {P,\left\{ {{{\tilde P}^{\left( m \right)}},{Q^{\left( m \right)}}} \right\}_{m = 1}^l,\gamma } \right)} f\left( {P,\sum\limits_{m = 1}^l {\gamma _m^2{{\tilde P}^{\left( m \right)}}{Q^{\left( m \right)}}} } \right)\\
{\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt} {\kern 1pt}  + \varphi \left( {P,\left\{ {{{\tilde P}^{\left( m \right)}},{Q^{\left( m \right)}}} \right\}_{m = 1}^l,\gamma } \right),
\end{array}
\end{equation}
where function $f$ is generally set as a trace operation in the above-mentioned works. ${Q^{\left( m \right)}}$ can be regarded as the perturbation matrix of the $m$-th modality. $\phi \left( {P,\left\{ {{{\tilde P}^{\left( m \right)}},{Q^{\left( m \right)}}} \right\}_{m = 1}^l,\gamma } \right)$ denotes the boundary constraint for these variables while $\varphi \left( {P,\left\{ {{{\tilde P}^{\left( m \right)}},{Q^{\left( m \right)}}} \right\}_{m = 1}^l,\gamma } \right)$ are the regularization constraints for these variables. In many works,  ${\tilde P^{\left( m \right)}}$ is the recovered complete representation for the $m$-th modality, where some rows of ${\tilde P^{\left( m \right)}} \in {R^{n \times c}}$ corresponding to the available modalities are fixed as the original initialized ${\bar P^{\left( m \right)}}$.

For the above late fusion based kernel methods, we can observe that: (1) These methods can simultaneously recover the modal-specific missing representations and learn the consensus representation by exploring the partially aligned structure information of data. (2) The performance of these methods highly relies on the quality of the initialized incomplete basis representations derived from the incomplete kernels.

\subsubsection{Deep learning based}
Recent years, deep learning received lots of attention in incomplete multimodal learning. For instance, Zhao \emph{et al}.~\cite{zhao2018incomplete} proposed a deep partial multimodal clustering network, which first uses deep encoders to extract the latent features of multimodal data and then adopts the graph regularized partial multimodal clustering model to learn the consensus representation from the incomplete bi-modal data. For data with more than two modalities, Wen \emph{et al}.~\cite{wen2020dimc} proposed several deep incomplete multimodal clustering networks based on deep autoencoder framework, cognitive learning \cite{2020CDIMC}, and graph neural network \cite{wen2021structural}, respectively. The objective function of these methods can be unified as the following formula:
\begin{equation}\label{im_eq6}
\min \sum\limits_{m = 1}^l {f\left( {{X^{\left( m \right)}},{{\bar X}^{\left( m \right)}}} \right)}  + {\lambda}g\left( {Z,\left\{ {{Z^{\left( m \right)}}} \right\}_{m = 1}^l} \right),
\end{equation}
where ${X^{\left( m \right)}} \in {R^{n \times {d_m}}}$ and ${\bar X^{\left( m \right)}} \in {R^{n \times {d_m}}}$ denote the original and reconstructed $m$-th modal data. $n$ denotes the number of samples and ${d_m}$ is the feature number of the $m$-th modal sample. ${W^{\left( m \right)}} \in {\left\{ {0,1} \right\}^{n \times n}}$ is a diagonal binary matrix as defined in (\ref{im_eq3}) to indicate the location of the missing modalities. $\bar Z$ and $\left\{ {{Z^{\left( m \right)}}} \right\}_{m = 1}^l$ represent the consensus or fused latent representation and the modal-specific latent representation at one layer of the network. ${\lambda}$ is penalty parameter. $f$ and $g$ are functions or constraints for these variables. For example,  $f$ is set as the mean square error (MSE) loss function in many methods. Objective (\ref{im_eq6}) can be also split into two independent losses to optimize two networks separately, where the first loss with the function $f$ is generally used for network pre-training. Similar to these unsupervised multimodal learning methods, Liu \emph{et al}. \cite{liu2023dicnet} developed an incomplete multimodal multi-label classification network, with the autoencoder based framework and multimodal contrastive constraint.

The above methods focus on the observed instances to train the network and can flexibly handle all kinds of incomplete data with more than two modalities by introducing the location matrix ${W^{\left( m \right)}}$ as prior weight in function $f$. In addition, a common technique adopted in these three methods is the weighted latent representation fusion, in which the location information of missing modalities is adopted as fusion weight to reduce the negative influence of missing modalities. Lately, Xu \emph{et al}.~\cite{xu2022deep} proposed an imputation-free and fusion-free deep network for incomplete multimodal data clustering. The method mines the multimodal cluster complementarity in the subspace and transforms such complementary information as supervised information to guide the network training. However, this method needs a part of samples with fully observed modalities for model training.

For supervised learning tasks, a incomplete multimodal learning framework is proposed in \cite{zhang2019cpm}, which can flexibly learn a common representation for arbitrary missing data and preserve both common and complementary information. For the more difficult task with incomplete labels, a deep double incomplete multimodal multi-label learning network~\cite{wen2023deep} is proposed. This deep network mainly introduces two mask constraints \textit{w.r.t.} the missing view locations and missing label locations, to reduce the negative impact of the missing labels and missing views. A good property of the method is that it can handle all kinds of incomplete data classification tasks including supervised/semi-supervised cases, complete/incomplete data, and complete/incomplete label cases. More recent work~\cite{mckinzie2023robustness} focuses on an even more generalized scenario than incomplete multimodal learning which is so called \textit{train-test modality mismatch}, where the test multimodal data can contains more or less modalities than training data. Specifically, all modalities are available at pretraining stage, while a completely different subset is encountered by the model during supervised training and testing in downstream tasks.

In medical image processing, Sanaz \textit{et al.} proposed MMCFormer~\cite{karimijafarbigloo2024mmcformer}, a novel missing modality compensation network to address the incomplete modalities for brain tumor segmentation. The proposed method is build upon 3D efficient transformer blocks and uses a co-training strategy to effectively train a missing modality network by ensuring feature consistency between complete modalities and incomplete modalities. Yao \textit{et al.} proposed DrFuse~\cite{yao2024drfuse} for effective medical diagnosis and forecasting prognosis with incomplete multimodal data. DrFuse first learns the common features shared between all modalities and modality-specific features within each separated modality and then weight and then combining the prediction from each modality to make the final prediction. Specifically, a disease-wise attention layer is devised to produce the patient- and disease-wise weights to tackle the modality inconsistency issue.

Some representative incomplete multimodal learning methods are summarized in Table 4.

\subsection{Discussion}
To sum up, the ways to handle incomplete data can be commonly divided into two categories, imputation-based incomplete multimodal learning and imputation-free incomplete multimodal learning. Methods that focus on imputing incomplete modalities can be classified into two types: one indirectly recovers the missing modalities through graph or kernel completion, and the other directly fills in the original data.
For imputation-free incomplete multimodal learning methods, their design philosophy focuses more on utilizing available modalities to explore information and understand multimodal data. However, both types of methods for handling incomplete multimodal data face deeper challenges. For example, the quality assessment of imputed instances for missing modalities is commonly overlooked. Besides, using prior missing information to mask unknown modalities is itself difficult to bridge the information gap and information imbalance issues caused by modal missing. Moreover, incomplete cases such as unpaired views \cite{wang2022lung,yu2020flexible,wang2024partially} and partially missing labels \cite{xing2021weakly} also need more attention. 
\input{incomplete/incomplete-table}

==> incomplete/taxon-table2.tex <==
\begin{table*}[htbp]
\setlength{\abovecaptionskip}{0.0cm}  %段前
\setlength{\belowcaptionskip}{0.0cm} %段后
\vspace{-0.0cm}
% \vskip 0.35in
\begin{center}
%\begin{spacing}{1.05}
\center\resizebox{0.99\textwidth}{!}{
{
\setlength{\tabcolsep}{1.9mm}
\begin{tabular}{c|c|c|c|c}
\toprule
  \multirow{1}{*}{\textbf{Category}}    &\multirow{1}{*}{\textbf{Reference}}   & \multirow{1}{*}{\textbf{Base model}} &
\multirow{1}{*}{\textbf{Learning Task}} & \multirow{1}{*}{\textbf{Applicable Data Forms}}
\\
\midrule

\multirow{2}{*}{Learning-free imputation} &  \cite{shao2015multiple},\cite{shao2016online}      &Weighted matrix factorization & Clustering & Arbitrary incomplete multi-modal data
            \\ \midrule
   &  \cite{wang2019spectral},\cite{gao2016incomplete}, \cite{zhou2019consensus}   &Graph learning (spectral clustering) & Clustering & Arbitrary incomplete multi-modal data
            \\ \midrule
 \cite{trivedi2010multiview}   &Learning based imputation    &Kernel learning with kernel element imputation & Clustering & Incomplete multi-modal data with two modalities and one complete modality
 \\ \midrule
  \cite{shao2013clustering}   &Learning based imputation    &Kernel learning with kernel element imputation & Clustering & Incomplete multi-modal data with two modalities
            \\ \midrule
  \cite{bhadra2017multi}, \cite{liu2019multiple}, \cite{zhu2018localized}, \cite{liu2021incomplete}   &Learning based imputation    &Kernel learning with kernel element imputation & Clustering & Arbitrary incomplete multi-modal data
            \\ \midrule
  \cite{wen2020adaptive}   &Learning based imputation    &Graph learning with graph element imputation & Clustering & Arbitrary incomplete multi-modal data
            \\ \midrule
  \cite{shang2017vigan}     &Learning based imputation    &Deep learning with raw data imputation & Missing modality generation & Incomplete multi-modal data with two modalities
  \\ \midrule
  \cite{wang2018partial} &Learning based imputation    &Deep learning with raw data imputation & Clustering & Incomplete multi-modal data with two modalities
    \\ \midrule
  \cite{xu2019adversarial} &Learning based imputation    &Deep learning with raw data imputation & Clustering & Incomplete multi-modal data with some paired samples

    \\ \midrule
  \cite{arya2021generative} &Learning based imputation    &Deep learning with raw data imputation & breast cancer prediction & Incomplete multi-modal data with some paired samples
  
  \\ \midrule
\cite{tran2017missing},\cite{tang2022deep} &Learning based imputation    &Deep learning with raw data imputation & Missing modality generation & Arbitrary incomplete multi-modal data
  \\ \midrule
  \cite{Liu2023Information}&Learning based imputation    &Deep learning with feature imputation & Missing modality generation & Arbitrary incomplete multi-modal data
  \\ \midrule

\cite{wen2019unified},\cite{yin2021incomplete} &Learning based imputation    &Matrix factorization with raw data imputation & Clustering & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{wen2021unified} &Learning based imputation    &Matrix factorization, tensor learning and graph element imputation & Clustering & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{li2014partial},\cite{zhao2016incomplete},\cite{xu2018partial} &Imputation-free    &Matrix factorization & Clustering & Incomplete multi-modal data with two modalities
  \\ \midrule
\cite{hu2018doubly},\cite{hu2019one} &Imputation-free    &Weighted matrix factorization & Clustering & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{deng2023projective} &Imputation-free    &Projection learning & Clustering & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{li2021concise} &Imputation-free    &Weighted projection learning & Classification & Arbitrary incomplete multi-modal multi-label data
  \\ \midrule
\cite{xiang2013multi}&Imputation-free    &Linear regression & Alzheimer's disease prediction & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{zhou2019latent}&Imputation-free    &Latent representation learning and linear regression & Alzheimer's disease diagnosis & Incomplete multi-modal Neuroimaging and Genetic data with special incomplete case
  \\ \midrule
  \cite{wu2018incomplete} &Imputation-free    &Graph learning & Clustering & Incomplete multi-modal data with two modalities
  \\ \midrule
\cite{wen2018incomplete}, \cite{wen2023highly} &Imputation-free    &Graph learning & Clustering & Arbitrary incomplete multi-modal data
 \\ \midrule
\cite{liu2017view} & Imputation-free    &Graph learning & Alzheimer's disease diagnosis & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{liu2018late}, \cite{liu2020efficient}, \cite{zhang2021one}  &Imputation-free    &Kernel learning & Clustering & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{zhao2018incomplete}  &Imputation-free    &Deep learning and matrix factorization & Clustering & Incomplete multi-modal data with two modalities
  \\ \midrule
\cite{2020CDIMC}, \cite{wen2021structural}, \cite{xu2022deep}  &Imputation-free    &Deep learning with weighted representation fusion & Clustering & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{zhang2019cpm}  &Imputation-free    &Representation learning & Classification & Arbitrary incomplete multi-modal data
  \\ \midrule
\cite{wen2023deep}  &Imputation-free    &Deep learning with weighted fusion and weighted loss & Classification & Arbitrary incomplete multi-modal multi-label data
%  \\ \midrule
  
                                                                                   \\ 
                                                                                   \bottomrule
\end{tabular}}}
% \end{spacing}
\end{center}
\end{table*}


==> noise/noise_backup.tex <==
\section{Learning on Noisy Multimodal Data}
Collecting high-quality multimodal data in real-world scenarios inevitably faces significant challenges due to the presence of noise. Multimodal data \cite{kulkarni2020pixel} noise can arise from sensor errors~\cite{DBLP:conf/cvpr/ChengZDJL19}, environmental interference, or transmission losses. For vision modality, the electronic noise in sensors leads to detail loss. Besides, audio modality may suffer from unexpected distortion due to environmental factors. To make things worse, weakly aligned or even unaligned multimodal samples are also commonly presented, which can be seen as more complex noise that lies in a higher-level semantic space. Fortunately, considering the correlation between multiple modalities or better utilizing multimodal data can help the fusion of noisy multimodal data. Various related works \cite{salvi2023multi,DBLP:conf/cvpr/BaiHZHCFT22,DBLP:conf/cvpr/ChengZDJL19} demonstrate that multimodal models surpass their unimodal counterparts. This can be attributed to the ability of multimodal data to identify and mitigate potential noise by leveraging the correlations among different modalities.

Multimodal noise can be roughly split into two categories according to their source: 1) modal-specific noise that arises from sensor errors, environmental factors, or transmission of each modality separately, 2) cross-modal noise that arises from weakly aligned or unaligned multimodal pairs which can be regarded as semantic level noise.

\subsection{Modal-specific noise reduction} 
Modal-specific noise reduction methods highly depends on the input modalities and task at hand. In this section, we focus on \textbf{visual} noise reduction in multimodal image fusion task to present a showcase. Most modal-specific denoise methods focus on aggregating useful information from multimodal data and mitigating the influence of noise in multimodal fusion.

\subsubsection{Weighted average fusion}
A simple multimodal noise reduction way is to conduct average fusion over multimodal data. Due to the randomness of noise, the average operation effectively reduces the noise in fused images. Rajalingam \emph{et al.} \cite{rajalingam2022intelligent} developed an intelligent multimodal fusion algorithm. The method decomposes the input image into high-frequency and low-frequency components and proposes an average fusion rule for the low-frequency components while utilizing guided filtering for the high-frequency components. Essentially, average-based multimodal noise reduction methods assign the same fusion weights to different modalities. However, the noise severity of each modality is different and varies among multimodal samples. To address the aforementioned issue, weighted average-based multimodal noise reduction method is proposed. Budhiraja \emph{et al}. \cite{budhiraja2015multimodal} proposed a multimodal image fusion scheme based on the guided filter. Their approach involves Gaussian decomposition with local average energy and average gradient-based salient maps for the base layer and detail layer, respectively. Qu \emph{et al}. \cite{qu2001medical} proposed a fusion rule used for calculating the wavelet transformation modulus maxima of input images with different bandwidths and levels. The approach aims to effectively combine the information from multiple image modalities. Achim \emph{et al}.\cite{achim2005complex} developed a fusion rule based on fractional lower-order moments for magnetic resonance (MR) and Computed Tomography (CT) images in the multi-scale medical image analysis literature. Considering the similarities and disparities between the different modalities,  Yu \emph{et al}.~\cite{yu2011image} divided the image into the common component and innovation component and represented the source image with the common and innovation sparse coefficients by joint sparse representation. Wang \emph{et al}. \cite{DBLP:journals/inffus/GogateDAH20} designed a gate mechanism to dynamically fuse visual features. By utilizing visual features as supplementary information, the proposed method effectively mitigates the influence of noise in voice signals. However, this strategy assumes that the visual data is clean. If the visual data is also corrupted by noise, this solution may be sub-optimal. Sadeghi \emph{et al}. \cite{DBLP:conf/icassp/SadeghiA21} adopted a latent sequential variable with Markovian dependencies to decide whether visual data is beneficial to audio-visual speech enhancement. Bai \emph{et al}.\cite{DBLP:conf/cvpr/BaiHZHCFT22} proposed a soft-association mechanism to handle inferior image conditions. In practice, the self-attention in Transformer can be used to adaptively decide where and what information should be taken from the image. Cheng \emph{et al}. \cite{DBLP:conf/cvpr/ChengZDJL19} adopted both soft attention and hard attention to mitigate noise issue, which is caused by rolling-shutter effect in lidar-stereo fusion task. Specifically, a fusion block is utilized to aggregate supplement information from stereo cameras and generates two disparity maps. Then, by comparing disparity map and lidar point, the noisy points in raw data are filtered out.

\subsubsection{Joint variation based fusion}
Joint optimization is often used in variation-based noise reduction when fusing multiple visual modalities, e.g., RGB and thermal. In unimodal noise reduction field, taking image modality as an example, classical denoise model based on Total Variation (TV) is equivalent to solving the following optimization problems:
\begin{equation}
   \min  \iint\left [ u(x, y) - u_0(x, y) \right ] ^2dxdy + \lambda \iint \left | \bigtriangledown u(x, y)  \right |  dxdy,  
\end{equation}
where $u_0(x, y), u(x, y)$ represent the input pixel and output pixel after noise reduction respectively. For multimodal noise reduction, the joint variational model for fusion and denoise is defined as follows:
\begin{equation}
    \min  \iint \sum_{m = 1}^{M} w_m \left [ u(\boldsymbol{x} ) - u_m(\boldsymbol{x} ) \right ] ^2d\boldsymbol{x} + \lambda \iint \left | \bigtriangledown u(\boldsymbol{x} )  \right |  d\boldsymbol{x},  
\end{equation}
where $u_m(\boldsymbol{x} )$ represents the input data from modality $m$, $w_m$ is the non-negative weight satisfying $\sum_{m = 1}^{M}w_m=1$. In a nutshell, joint optimization is the solution of a specific optimization problem using data from different modalities. Wang \emph{et al}. \cite{wang2008variational} proposed a variational model in the pixel domain and wavelet domain for joint fusion and denoise of noisy multifocus images. Kumar \emph{et al}. \cite{kumar2009total} also employed the total variational model to fuse images acquired using multiple sensors and achieves excellent results on two modal images provided in the medical field and aircraft navigation field. Recently, Padmavathi \emph{et al}. \cite{padmavathi2020novel} proposed an image fusion algorithm for constructing a fused image using the total variation model. They incorporated an optimized adaptive weighting fusion scheme for medical multimodal data analysis (i.e., Magnetic Resonance images and Positron Emission Tomography images). Nie \emph{et al}. \cite{nie2021total} introduced a total variation-based fusion method for infrared and visible images. The method leverages the total variation model to fuse two modalities, enabling enhanced image quality and information integration. Quan \emph{et al}. \cite{quan2021relative} developed a feature fusion method called relative total variation structure analysis (RTVSA) for urban area classification. This approach combines various features derived from hyperspectral imaging (HSI) and LiDAR data, providing a comprehensive analysis for accurate classification. Furthermore, Liu \emph{et al}. \cite{liu2022tse_fuse} designed a two-stage enhancement (TSE) framework for infrared and visible image fusion. Their framework incorporated an attention mechanism and a feature-linking model (FLM), combining structure adaptive total-variational (SATV) and L1 sparsity terms to extract two-scale detail layers and a base layer. The proposed method demonstrates robustness and effectiveness in improving the quality of fused images.

\subsection{Cross-modal noise reduction}
Many multimodal tasks (e.g., multimodal object detection, vision-and-language understanding) highly depends on correctly aligned multimodal training data. However, the real-world multimodal pairs tend to contain weakly aligned or even unaligned samples~\cite{changpinyo2021conceptual}. For example, in RGB-thermal multimodal object detection, multimodal inputs are often weakly aligned, i.e., the locations of the same objects may be shifted across different modalities~\cite{zhang2019weakly}. In social media, the text descriptions are frequently irrelevant with the image content, i.e., unpaired modalities. In this section, we consider weakly aligned or unaligned multimodal samples as cross-modal noise. Compared to modal-specific noise, cross-modal noise lies in a higher-level semantic space. Current cross-modal noise reduction methods can be roughly split into rules-based filtering, model-based rectifying and noise robustness regularization.

From the data perspective, some strict rules are used to conduct data cleaning~\cite{sharma-etal-2018-conceptual, radenovic2023filtering, gadre2023datacomp}. As a recent representative method, CAT (Complexity, Action, and Text-spotting) is a filtering strategy which is devised to select informative image-text pairs, thereby reducing the influence of cross-modal noise~\cite{radenovic2023filtering}.  In multi-spectral  object detection, image registration (i.e., spatial alignment) is a commonly used pre-processing~\cite{maintz1998survey,zitova2003image}. By employing geometric rules to align two images, the shifted positions can be rectified across different modalities.

From the model perspective, model filtering or rectifying methods try to identify cross-modal noise samples and further remove or rectify them. To achieve this, Huang \emph{et al}. proposed a method called Noisy Correspondence Rectifier (NCR) to tackle cross-modal noise~\cite{huang2021learning}. NCR leverages the memorization effect of neural networks, dividing the data into clean and noisy subsets based on loss differences. Subsequently, it rectifies correspondence using an adaptive prediction model in a co-teaching manner. Applied to image-text matching as a showcase, NCR achieves superior performance in the presence of cross-modal noisy data. ALBEF~\cite{li2021align} adopts momentum models to generate pseudo targets as additional supervision. BLIP~\cite{li2022blip} introduces a filter to remove the noisy data according to the similarity of image-text pairs and then utilizes a captioner to regenerate the corresponding web texts. This filtering and captioning strategy can improve the quality of multimodal pairs, contributing to the improvement of downstream vision-language tasks.

Noise robust regularization is another perspective to mitigate the influence of cross-modal noise. To explicitly stabilize and harmonize multimodal pretraining and mitigate the influence of latent noise, NLIP~\cite{huang2023nlip} employs noise-adaptive regularization to avoid overfitting to noisy image-text pairs, adjusting alignment labels based on estimated noisy probabilities. Additionally, NLIP utilizes a concept-conditioned cross-modal decoder to generate synthetic captions to impute the missing object information. To mitigate the influence of cross-modal noise in vision-language task, Li \emph{et al}.~\cite{li2020oscar} proposed OSCAR that detects object tags in images and uses them as anchor points for alignment. Recent work provides both theoretical and empirical analysis to shed light on the influence of cross-modal noise in multimodal contrastive learning~\cite{nakada2023understanding}. Furthermore, the research introduces a novel MMCL loss designed to handle unpaired multimodal samples, demonstrating enhanced robustness in empirical experiments.

\subsection{Discussion}
To summarize, learning from noisy multi-modal data is a common but challenging problem. Current approaches address this problem from two perspectives: modal-specific noise reduction (for feature noise) and cross-modal noise reduction (for semantic noise). However, these methods typically focus on specific scenarios, such as multimodal image fusion or automatic driving, leaving the exploration of general noise patterns and learning paradigms relatively unexplored. We have identified several potential research topics in this field. First, it is important to leverage the correlation between noises in different modalities. For instance, images with similar wavelengths in a hyper-spectral image often exhibit similar noise patterns. Second, it will be effective to leverage the complementarity between noisy and clean modalities for noise reduction. Third, addressing high-level semantic noise poses an interesting direction and it is more challenging. For example, how can we tackle this problem using Multimodal Large Language Models (MLLM)?
\input{table/noise}

==> table/feature-noise.tex <==
\begin{table*}[ht]
\centering
\caption{A summary of representative multi-modal feature noise reduction works.}
\begin{adjustbox}{max width=1\textwidth}
\begin{tabular}{@{}|c|c|c|c|@{}}
\toprule
\textbf{Reference} & \textbf{Fusion Paradigm} & \textbf{ Model-specific}  & \textbf{Application}                           \\ 
        \midrule

        \cite{achim2005complex}    & Weighted fusion & Filter based  &  Image fusion \\
        
        \cite{budhiraja2015multimodal}    & Weighted fusion & Filter based   &  Image fusion \\
        
        \cite{rajalingam2022intelligent}   & Average fusion  & Filter based   &  Image fusion \\  
        
        \cite{DBLP:journals/inffus/GogateDAH20} \cite{DBLP:conf/icassp/SadeghiA21}   &Weighted average  &Deep learning based  & Audio enhancement \\
        
        \cite{DBLP:conf/cvpr/BaiHZHCFT22}   &Weighted average  &Deep learning based & Object detection \\
        
        \cite{DBLP:conf/cvpr/ChengZDJL19}    &Weighted average  &Deep learning based  & Lidar-stereo fusion \\
        
        \cite{DBLP:conf/iros/EitelSSRB15}    &Weighted average  &  Deep learning based  & RGB-D object recognition \\
            
        \cite{hong2020x} &Weighted average  &Deep learning based  & Image classification \\
        
        \cite{DBLP:journals/tec/HuangJB21}   &Weighted average  & Deep learning based  & Multi-modal representation learning \\
        
    \midrule
    
        \cite{qu2001medical}    & Average and maximum fusion & Filter based  &  Image fusion \\
        
        \cite{singh2009multimodal}    & Maximum entropy fusion & Filter based &  Image fusion \\
        
        \cite{singh2014fusion}    & Maximum selection fusion & Filter based &  Image fusion \\

    \midrule

        \cite{kumar2009total}     & Joint optimization & Variation based &  Image fusion \\
        
        \cite{zhao2017medical}   & Joint optimization  & Variation based & Medical image fusion  \\
        
        \cite{padmavathi2020novel} & Joint optimization & Variation based &  Image fusion \\
        
        \cite{nie2021total}   & Joint optimization & Variation based &  Image fusion \\
        
        \cite{quan2021relative}    & Joint optimization & Variation based & Classification and remote sensing \\
        
        \cite{liu2022tse_fuse}    & Joint optimization & Variation based &  Image fusion \\

    \midrule
         \cite{yu2011image}  & Weighted average& Factorization based  &  Image fusion and denoising \\
        \cite{yang2009multifocus} &  Choose-max& Factorization based &  Image fusion and denoising \\
        
       \cite{li2018joint}  & Choose-max & Factorization based  &  Image fusion and denoising\\
       
       
        
   
        


        %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \midrule
    
%         \cite{DBLP:journals/inffus/GogateDAH20} \cite{DBLP:conf/icassp/SadeghiA21}   &Weighted average Deep learning based &  & Fusion and  denoising & Audio enhancement \\
%         \cite{DBLP:conf/cvpr/BaiHZHCFT22}   &Weighted averag Deep learning based &e & Fusion and denoising  & Object detection \\
%         \cite{DBLP:conf/cvpr/ChengZDJL19}    &Weighted average Deep learning based &  &  Fusion and denoising & Lidar-stereo fusion \\
%         \cite{DBLP:conf/iros/EitelSSRB15}
%             &Weighted average  Deep learning based &  &  Denoising  & RGB-D object recognition \\
%         \cite{hong2020x} &Weighted average Deep learning based &  & Fusion and denoising & Image classification \\
%         \cite{DBLP:journals/tec/HuangJB21}   &Weighted average Deep learning based &  &  Fusion and denoising  & Multi-modal representation learning \\
%     \midrule
%         \cite{budhiraja2015multimodal}    & Weighted fusion & Filter based & Fusion  &  Image fusion \\
%         \cite{rajalingam2022intelligent}   & Average fusion  & Filter based & Fusion  &  Image fusion \\
%         \cite{qu2001medical}    & Average and maximum fusion & Filter based & Fusion  &  Image fusion \\
%         \cite{achim2005complex}    & Weighted fusion & Filter based & Fusion  &  Image fusion \\
%         \cite{singh2009multimodal}    & Maximum entropy fusion & Filter based & Fusion  &  Image fusion \\
%         \cite{singh2014fusion}    & Maximum selection fusion & Filter based & Fusion  &  Image fusion \\

%     \midrule

% %        \cite{wang2008variational}     & Variation based & Joint optimization & Fusion and denoising  & Image fusion and denoising  \\
%         \cite{kumar2009total}     & Joint optimization & Variation based & Fusion  &  Image fusion \\
%         \cite{zhao2017medical}   & Joint optimization  & Variation based & Fusion and denoising  & Medical image fusion  \\
% %        \cite{mei2019simultaneous}    & Variation based & Joint optimization & Fusion and denoising  & Image fusion and denoising  \\
% %        \cite{zhao2019ct}   & Variation based & Joint optimization& Fusion  &  Image fusion \\
%         \cite{padmavathi2020novel} & Joint optimization & Variation based & Fusion  &  Image fusion \\
% %        \cite{liu2020robust}    & Variation based & Joint optimization & Fusion  &  Image fusion \\
%         \cite{nie2021total}   & Joint optimization & Variation based & Fusion  &  Image fusion \\
% %        \cite{yu2021adaptive}    & Variation based & Joint optimization & Subspace optimization  &  Sound source localization \\
%         \cite{quan2021relative}    & Joint optimization & Variation based & Fusion  & Classification and remote sensing \\
%         \cite{liu2022tse_fuse}    & Joint optimization & Variation based & Fusion  &  Image fusion \\

%     \midrule
        
%         \cite{yang2009multifocus} & Choose-max & Factorization based &  Fusion &  Image fusion and denoising \\
        
%         \cite{yu2011image}  & Weighted average & Factorization based & Fusion  &  Image fusion and denoising \\
        
%         \cite{li2018joint}  & Choose-max & Factorization based & Fusion  &  Image fusion and denoising\\
        
%         \cite{li2019discriminative}    & Sum-modified-llaplacian & Factorization based & Fusion  &  Image fusion and denoising \\

%     % \midrule
    
%     %     \cite{DBLP:journals/inffus/GogateDAH20}    & deep learning based & Fusion and  Denoising & Audio enhancement \\
%     %     \cite{DBLP:conf/icassp/SadeghiA21}   & deep learning based & Fusion and  Denoising  & Audio enhancement \\
%     %     \cite{DBLP:conf/cvpr/BaiHZHCFT22}   & deep learning based & Fusion and Denoising  & Object detection \\
%     %     \cite{DBLP:conf/cvpr/ChengZDJL19}    & deep learning based &  Fusion and Denoising & Lidar-stereo fusion \\
%     %     \cite{DBLP:conf/iros/EitelSSRB15}
%     %     \cite{hong2020x}    & deep learning based &   &  \\
%     %     \cite{DBLP:journals/tec/HuangJB21}   & deep learning based &   &  \\
        
%     % \bottomrule

        
    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> table/label-noise.tex <==
\begin{table*}[ht]
\centering
\caption{A summary of representative multi-modal label noise reduction works.}
\begin{tabular}{@{}|c|c|c|c|@{}}
\toprule
\textbf{Reference} & \textbf{Problem} & \textbf{Method category}              & \textbf{Application}                           \\ \midrule
      \cite{mandal2020cross}     & Explicit MLNR & correcting the wrong label based      & cross-modal retrieval                          \\
      \cite{cheng2022joint}    & Explicit MLNR & removing the wrong label based        &audio-visual video parsing \\
      \cite{wu2021exploring}    & Explicit MLNR & correcting the wrong label based      & audio-visual video parsing                     \\
      \cite{DBLP:conf/cvpr/00020ZZ021}   & Explicit MLNR & learning objective based              & cross-modal retrieval                          \\
      \cite{wang2021noise}   & Explicit MLNR & training strategy based               & cross-modal hashing                            \\
      \cite{gan2023collaborative}     & Explicit MLNR & training strategy based               & multi-modal highlight detection                \\ \midrule
      \cite{huang2021learning},\cite{huang2021learning},\cite{DBLP:conf/mm/QinP00022}    & Implicit MLNR  & generating soft alignment label based & cross-modal retrieval                          \\
      \cite{DBLP:conf/nips/LiSGJXH21},    & Implicit MLNR  & generating soft alignment label based & language-vision pretraining                    \\
      \cite{DBLP:journals/corr/abs-2212-13563}   & Implicit MLNR  & learning objective based              & image captioning                               \\
      \cite{DBLP:journals/corr/abs-2212-07086}    & Implicit MLNR  & learning objective based              & language-vision pretraining                    \\
      \cite{thomas2022emphasizing}    & Implicit MLNR  & training strategy based               & cross-modal retrieval                          \\ \bottomrule
\end{tabular}
\end{table*}

==> table/noise_backup.tex <==
\begin{table*}[ht]
\centering
\caption{A summary of representative multi-modal noise reduction works.}
\begin{adjustbox}{max width=1\textwidth}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\toprule
\textbf{Noise type} & \textbf{Reference} & \textbf{Denoise Paradigm} & \textbf{Application}                           \\ 
        \midrule
        
      &  \cite{rajalingam2022intelligent}   & Average fusion  &  \multirow{3}{*}{Image fusion} \\ \cline{2-3}

    \multirow{14}{*}{Modal-specific} & \cite{achim2005complex}    & \multirow{8}{*}{Weighted fusion} &   \\
        
      &  \cite{budhiraja2015multimodal}    &   &   \\ \cline{4-4}  
        
      &  \cite{DBLP:journals/inffus/GogateDAH20} \cite{DBLP:conf/icassp/SadeghiA21}   &  & Audio enhancement \\ \cline{4-4} &
        
        \cite{DBLP:conf/cvpr/BaiHZHCFT22}   &  & Object detection \\\cline{4-4} &
        
        \cite{DBLP:conf/cvpr/ChengZDJL19}    &  & Lidar-stereo fusion \\ \cline{4-4} &
        
        \cite{DBLP:conf/iros/EitelSSRB15}    &  & RGB-D object recognition \\ \cline{4-4} &
            
        \cite{hong2020x} &  & Image classification \\\cline{2-2} \cline{4-4} &
        
        \cite{DBLP:journals/tec/HuangJB21}   &  & Representation learning \\ \cline{2-4} &

    

        \cite{kumar2009total}     & \multirow{6}{*}{Joint variation} &\multirow{6}{*}{Image fusion}   \\ \cline{2-2}   &
        
        \cite{zhao2017medical}   &   &  \\ \cline{2-2}   &
        
        \cite{padmavathi2020novel} &  &   \\ \cline{2-2}   &
        
        \cite{nie2021total}   &  & \\ &
        
        \cite{liu2022tse_fuse}    &  &    \\ \cline{2-2}  \cline{4-4} &
        
        \cite{quan2021relative}    &  & Remote-sensing scene classification  \\ \midrule \multirow{5}{*}{Cross-modal} & \cite{sharma-etal-2018-conceptual, radenovic2023filtering, gadre2023datacomp}
        
         &\multirow{1}{*}{Rules-based filtering}  & \multirow{1}{*}{Multimodal pretraining}   \\\cline{2-4}  &\cite{huang2021learning} 
        
         &\multirow{2}{*}{Model-based rectifying}  &Image-text matching   \\ \cline{2-2} \cline{4-4}  &\cite{li2021align,li2022blip} 
        
         &  &Multimodal pretraining \\\cline{2-4}  &\cite{huang2023nlip,nakada2023understanding} 
        
         &\multirow{2}{*}{Noise robust regularization}  &Multimodal pretraining   \\\cline{2-2} \cline{4-4}  &\cite{li2020oscar} 
        
         &  &Vision-language understanding   \\
       
        
   
        



        
    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> table/noise_backup241015.tex <==
\begin{table*}[ht]
\caption{A summary of representative multi-modal noise reduction works.}
\center\resizebox{0.99\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{Noise type} & \textbf{Denoise Paradigm} & \textbf{Application} & \textbf{Reference}                           \\ 
        \midrule
        
         & Average fusion  &  \multirow{3}{*}{Image fusion} &  \cite{rajalingam2022intelligent} \\ \cline{2-2} 

    \multirow{14}{*}{Modal-specific} & \multirow{8}{*}{Weighted fusion} & & \cite{achim2005complex}       \\
        
      &      &   & \cite{budhiraja2015multimodal}  \\ \cline{3-4}  
        
      &    & Audio enhancement &\cite{DBLP:journals/inffus/GogateDAH20} \cite{DBLP:conf/icassp/SadeghiA21}   \\ \cline{3-4} &
        
          & Object detection &  \cite{DBLP:conf/cvpr/BaiHZHCFT22}\\\cline{3-4} &
        
            & Lidar-stereo fusion &\cite{DBLP:conf/cvpr/ChengZDJL19}\\ \cline{3-4} &
        
            & RGB-D object recognition &\cite{DBLP:conf/iros/EitelSSRB15} \\ \cline{3-4} &
            
        & Image classification &\cite{hong2020x} \\\cline{3-4} &
        
          & Representation learning &\cite{DBLP:journals/tec/HuangJB21} \\ \cline{2-4}

    

           & \multirow{6}{*}{Joint variation} &\multirow{6}{*}{Image fusion} & \cite{kumar2009total}    \\ \cline{4-4}     &   & &
        
        \cite{zhao2017medical}  \\ \cline{4-4}    &  & &
        
        \cite{padmavathi2020novel}  \\ \cline{4-4}     &  & &
        
        \cite{nie2021total}  \\    &  &  &
        
        \cite{liu2022tse_fuse}   \\ \cline{3-3}  \cline{4-4}   &  & Remote-sensing scene classification &
        
        \cite{quan2021relative}   \\ \cline{1-4} \multirow{5}{*}{Cross-modal} 
        
         &\multirow{1}{*}{Rules-based filtering}  & \multirow{1}{*}{Multimodal pretraining} & \cite{sharma-etal-2018-conceptual, radenovic2023filtering, gadre2023datacomp}   \\\cline{2-4} 
         &\multirow{2}{*}{Model-based rectifying}  &Image-text matching  &\cite{huang2021learning} 
          \\ \cline{3-3} \cline{4-4} 
         &  &Multimodal pretraining  &\cite{li2021align,li2022blip} 
         \\\cline{2-4}  
         &\multirow{2}{*}{Noise robust regularization}  &Multimodal pretraining  &\cite{huang2023nlip,nakada2023understanding} 
         \\\cline{3-3} \cline{4-4}  
        
         &  &Vision-language understanding  &\cite{li2020oscar}  \\
       
        
   
        



        
    \bottomrule
\end{tabular}}
\end{table*}
